Similar Part Rearrangement With Pebble Graphs

This work proposes a method for effectively computing manipulation paths to rearrange similar objects in a cluttered space. The solution can be used to place similar products in a factory floor in a desirable arrangement or for retrieving a particular object from a shelf blocked by similarly sized objects. These are challenging problems as they involve combinatorially large, continuous configuration spaces due to the presence of multiple moving bodies and kinematically complex manipulators. This work leverages ideas from algorithmic theory, multi-robot motion planning and manipulation planning to propose appropriate graphical representations for this challenge. These representations allow to quickly reason whether manipulation paths allow the transition between entire sets of objects arrangements without having to explicitly enumerate the path for each pair of arrangements. The proposed method also allows to take advantage of precomputation given a manipulation roadmap for transferring a single object in the same cluttered space. The resulting approach is evaluated in simulation for a realistic model of a Baxter robot and executed in open-loop on the real system, showing that the approach solves complex instances and is promising in terms of scalability and success ratio.

==> 04_03_augment.tex <==
The generated pebble graphs only include edges which are completely 
collision-free.  This is rather restrictive, however, especially as 
more poses are considered within a single the pebble graph.  In order 
to alleviate this problem, the pebble graphs can be augmented to 
include additional edges between the poses.  These additional edges 
represent transitions that can be made assuming that some small 
rearrangement takes place in the existing connected components of the 
already constructed pebble graph.  This process can be applied 
iteratively, and is outlined in Algorithm \ref{algo:augment}.

\begin{figure}[ht]
  \centering
  \begin{tabular}{| c | c |}
    \hline
    Notation & Meaning \\
    \hline
    $\cons$ & A set of computed constraints. \\
    $\kedges$ & Set of edges with motion constraints. \\
    $\pi$ & Path for the robot manipulator. \\
    \hline
  \end{tabular}
  \caption{Relevant notation for augmenting pebble graphs.}
  \label{tab:augment_notation}
\end{figure}

At a high-level, the idea is that each edge which is not 
collision-free treats a collision with an object as a constraint.
These constraints are associated with each edge, as seen in Figure
\ref{fig:build_pumped} (c), and the algorithm checks whether it is
feasible to remove objects from the constraining locations.  If 
there are enough free locations and the objects can be rearranged 
along paths which have their constraints satisfied, then these new
edges can be added to the pebble graph.

\input{algo_augment}

In practice, this augmentation procedure can be done in-line with 
the origial creation of the pebble graph.  That is, if an edge is
found to be in collision in Algorithm \ref{algo:create_pumped}, the
constrained edges can automatically be created with their appropriate
constraints, as is done in Algorithm \ref{algo:augment} (Lines 4-7).
Then, the final loop for adding additional edges to the pebble 
graph can be run.


==> 05_01_manip_prm.tex <==
In order to generate paths in the environment, faster and not computing them online, that will allow the arm to grasp and move objects, the proposed methodology first constructs a variation of a manipulation roadmap $\roadmap( \nodes, \edges )$. The roadmap $\roadmap$ is constructed only for the manipulator and a single object while taking into account the static geometry.  In this manner, the roadmap operates over reduced collision-free single-object states of the form $x = ((q^{\Manip}, p),t)$, where $q^{\Manip} \in \Qspace^{\Manip}$ is a manipulator configuration, $p$ is the pose of the single object copy and $t$ is the type, i.e., either a transfer or a transit state.

The first step in the construction of $\roadmap$ is to sample transition
states $x^{t} \in \Xspace^{t}$, where the robot is in a grasping
configuration and the object is in a stable pose.  This can be
achieved by first sampling a stable collision-free object pose,
$p \in \Pspace^s$, and then using inverse kinematics to
define the corresponding manipulator's grasping configuration
$q^{\Manip}$ (as the configurations shown in
Fig. \ref{fig:transitions} for the Baxter robot). If the inverse
kinematics function returns a solution and the resulting configuration
$(q^{\Manip},p)$ is collision-free, then two states are generated with
the same configuration: one of the transit type and one of the
transfer type. Both of these states are inserted in the manipulation
roadmap and an edge is added in the roadmap for each such pair of
transition states.  

In the experiments performed for this paper multiple attempts to
generate grasping configurations for the manipulator take place for an
individual object pose. Furthermore, two extra states are inserted into 
the manipulation roadmap directly during this process. A transit state, will
be called retraction state, where the arm's end effector is slightly retracted 
from the object, and a transfer state, will be called raised state, where the 
arm's end effector is slightly raised with the object. These additional states
help in the connectivity of both the transit and transfer subsets of the 
manipulation roadmap.

Given the set of transition states and edges, the method proceeds to
explore separately the transit and the transfer subset of the state
space in a \prmstar\ fashion. For the transit component, additional
grasping configurations for the manipulator are sampled where the
object is no longer required to be in a stable pose. Then neighboring
transit states according to a configuration space metric are
considered for connection by interpolating between the two
configurations. If the interpolated path is collision-free, then the
corresponding edge is added to the roadmap. The same process is
repeated for transfer states. The objective is to achieve a roadmap that
has the minimum number of connected components, so that the
manipulator is able to transfer objects among the sampled transition
states.

After the roadmap is being constructed, still in the offline process, is getting informed for collisions with the poses of the $\roadmap$. All the sampled poses that have been used in order to build the manipulation roadmap, are checked for collisions with the edges of the roadmap. This information will be used during the online process in order to speed up the searches for collision free paths for the manipulator. 

\begin{figure*}
\centering
\includegraphics[width=2.2in]{figures/RPG1}
\hspace{0.1in}
\includegraphics[width=2.2in]{figures/RPG2}
\hspace{0.1in}
\includegraphics[width=2.2in]{figures/RPG3}
%\includegraphics[width=1.72in]{figures/pumpedd}
\caption{\rpg\ creation: a) The algorithm iteratively selects valid
$\nobj + \nblank$ stable grasps, from the set that has been used in
order to build the manipulation roadmap, and generates a pumped
arrangement.  b) For each pair of poses, the method adds an edge if it
is possible given the roadmap to transfer an object between these
poses (A to E) without collisions. If a collision with a potentially
placed object on another pose is detected, the method remembers this
as a constraint. Some of the edges with constraints may be
traversable. c) The new \rpg\ is returned with the collision free
edges and the constrained edges in a separate structure $\cedges$. }
\label{fig:build_pumped_graph}
\end{figure*}

Given this roadmap and the information about the poses that have been
used in order to build the roadmap, both the selection of the poses
for the \rpg\ and the edges in a \rpg, which correspond to a motion of
the manipulator that is moving an object from one pose to another, is
now easier. First the poses of the \rpg\ is been selected randomly
from the poses that used for the construction of $\roadmap$
(Fig.\ref{fig:build_pumped_graph}a). The roadmap has already multiple
configurations $q^{\Manip} \in \Qspace^{\Manip}$, where can grasp an
object in a stable configuration on that pose. In order to add an edge
to the \rpg\ a path, that connects the safe $\safe$ configuration of
the manipulator, an $x^{t}_{\pose} \in \Xspace^{t}$ transition state
for the one pose, an $x^{t}_{\pose'} \in \Xspace^{t}$ transition state
for the other pose, and back to $\safe$, has to be computed. The safe
$\safe$ configuration for the manipulator, though, is also a node in
the roadmap, $\safe \in \roadmap$. So the roadmap can be used in order
to compute this path. A minimum conflict algorithm runs, between all
the different configurations $q^{\Manip}$ for each pose, in order to
find the least constrained path, $\safe \rightarrow
x^{t}_{\pose} \rightarrow x^{t}_{\pose'} \rightarrow \safe$
(Fig.\ref{fig:build_pumped_graph}b).





\begin{comment}
\begin{figure}
\includegraphics[width=1.42in]{figures/manipa}
\includegraphics[width=1.42in]{figures/manipb}
\includegraphics[width=1.42in]{figures/manipc}
\includegraphics[width=1.72in]{figures/manipd}
\caption{An illustration of the method used to construct the
  manipulation roadmap.  a) The method begins by sampling a set of
  stable grasps for a single object in various poses.  b) After
  generating the set of stable grasps, the method attempts to connect
  these stable grasps into a single roadmap.  c) After creating the
  stable grasps, each grasping state is duplicated, only this time the
  manipulator has released the object.  Then, the states where the
  object is released are connected.  d) Finally, the algorithm
  iteratively adds new manipulator positions and valid transitions
  between them to ensure the supplied safe state, $\safe$, is in the
  sameconnected component as released objects positions.}
\label{fig:manipulate}
\end{figure}


Then, local paths between pairs of states are tested for collision,
and collision-free trajectories are added as edges to the roadmap
(Lines 4-8, Figure \ref{fig:manipulate} (b)).

Figure \ref{fig:manipulate} (a)
Algorithm \ref{algo:arrange_prm})

\begin{figure}[ht]
  \centering
  \begin{tabular}{| c | c |}
    \hline
    Notation & Meaning \\
    \hline
     & The manipulation roadmap. \\
    $\frnodes$ & Non-grasping states in $\roadmap$. \\
    $\fredges$ & Set of non-grasping transitions in $\roadmap$. \\
    $\grnodes$ & Set of grasping states in $\roadmap$. \\
    $\gredges$ & Set of grasping transitions in $\roadmap$. \\    
    \hline
    $\safe$ & Safe state for the robot manipulator. \\
    \hline
    $\local$ & Local path between positions. \\
    \hline
  \end{tabular}
  \caption{Relevant notation for constructing the manipulation roadmap.}
  \label{tab:manip_notation}
\end{figure}

Then, the algorithm takes all the states which represent stable 
grasps and generates new states where the object has been released 
(Line 9).  These states, as well as the edges between them ,are kept 
in a separate structure for connected components testing.  These 
released states are used to further expand upon the roadmap, and local 
connections are created (Lines 10-16, Figure \ref{fig:manipulate} 
(c)).  Note that in Line 12, the local path between a stable grasp 
state and the corresponding released state are directly added to the 
roadmap.  It is pertinent to note that the safe state, $\safe$, 
for the robot is included in the set of released states (Line 1).

%\input{algo_manip_prm}

Finally, the algorithm attempts to refine the roadmap such that the
set of released positions lie in a single connected component, by 
incrementally adding new random manipulator positions (Figure 
\ref{fig:manipulate} (d)).  This ensures that from any vertex 
in the roadmap, there exists some path in the roadmap from any vertex 
back to the safe position, $\safe$.
\end{comment}


==> 05_02_high_level.tex <==
The proposed approach, $\prxpump$, operates in a similar fashion to
tree sampling-based motion planners.  In particular, it operates 
much like the Expansive Spaces Tree ($\est$) approach.  $\prxpump$
selects a node from within it's planning tree structure uniform at
random.  Then, from this node, a seed of poses is used in an 
expansion step to generate multiple nodes, as detailed in 
Algorithm \ref{algo:create_hypernode}.  The method keeps doing this
until some pre-specified stopping criterion, such as reaching a goal
arrangement, or reaching a maximum time limit.  When the algorithm 
detects that a goal configuration can be reached, it must perform a 
query in order to retrieve a motion plan that satisfies the query.


%The proposed approach, $\prxpump$, can be utilized in two different
%ways.  The first expands a forest of trees to construct the hypergraph,
%while the other follows a roadmap-based approach. The $\prxpump$ 
%approach requires as input the start configuration for the objects, 
%$\config_{start}$ as well as a safe state for the manipulator, 
%$\safe$.  Then, there are again two ways to run each variant in 
%regards to goal configurations.  In the case 
%of arrangement planning, a clearly defined goal arrangment of the 
%objects, $\config_{goal}$ can be provided.  In such a scenario, the 
%tree-based variant can grow a bi-directional tree until a connection
%between the trees can be established, and the roadmap-based variant
%will build the roadmap until $\config_{start}$ and 
%$\config_{goal}$ are in the same connected component.  Alternatively, 
%if the robot is given some goal, such as being able to touch a 
%particular object in the scene (which in this case, will be encoded 
%as a static geometry in the scene), then each created node in the 
%hypergraph can be tested for whether the goal can be achieved.

%$\prxpump$ begins by first constructing an arrangement roadmap,
%$\graph$, which is a lazy roadmap for solving manipulation-based 
%motion queries.  Then, it creates hypernodes, for the 
%start and goals appropriately, and begins building the hypergraph.  
%Whenever a new hypernode is added to the graph, then the appropriate 
%node ID information is stored in $\graph$.

%\subsubsection{\prxpump\ as a Roadmap}

%When constructing the hypergraph in this fashion, the algorithm
%randomly samples new nodes which consist of a pebble graph and a 
%corresponding signature.  Then, it attempts to connect all pairs of 
%generated nodes, using the described connection strategy to prune
%out infeasible connections.  Then, if there is a known goal state,
%this will also be added to the roadmap, otherwise, each newly
%generated node must be tested if it satisfies the goal criteria.

%\subsubsection{\prxpump\ as a Tree}

%The algorithm iteratively chooses a random node from within the tree
%or forest of trees (in the case of bidirectional search when goal 
%states are defined).  When the method expands existing nodes to 
%create new nodes, it does so in a manner that ensures a connection 
%can be created between the newly generated node, and existing pebble 
%graphs in nodes already in the tree, i.e. that the generated node's 
%pebble graph has at least $\nrob$ common positions with some other
%node.  

%This expansion process is detailed in Algorithm
%\ref{algo:expand}.  Using the described pumped configuration 
%generator (Line 2), the method computes the possible signatures this
%pumped configuration can have (Line 3).  Then, the set of new nodes
%is generated (Lines 4,5).
%
%\input{algo_expand_node}



==> algo_augment.tex <==
\begin{algorithm}[ht]
\caption{${\tt AUGMENT\_PG} (\pumped=(\pnodes,\pedges),\sign, \nrob,\graph,\safe)$}
\label{algo:augment}
$\kedges \gets \emptyset$\;
\For{pairs $(\pnode, \pnode') \in \pnodes$, $\pnode \neq \pnode'$}
{
  $\pi \gets {\tt Compute\_Cycle\_Path}(\graph, \safe, \pnode, \pnode', \pnodes)$\;
  $\cons \gets {\tt Compute\_Collisions}(\pi, \pnodes)$\;
  \If{$|\cons| < |\pedges| - k$}
  {
  	$\kedges \gets \kedges \cup ((\pnode,\pnode'), \pi, \cons)$\;
  }
}
\While{New edges added to $\pedges$}
{
	\For{$\kedge \in \kedges$}
	{
		\If{${\tt Test\_Feasible}(\kedge, sign)$}
		{
      $\pnodes \gets \pnodes \cup {\tt Endpoints}(\kedge)$\;
      $\pedges \gets \pedges \cup \kedge$\;
      $\kedges \gets \kedges \setminus \kedge$\;
		}
	}
}
$\sign \gets {\tt Recompute\_Signature}(\sign, \pumped)$\;
return $\pumped$\;
\end{algorithm}


==> algo_connect.tex <==
\begin{algorithm}[ht]
\caption{${\tt CONNECT\_NODE} (\hgraph=(\hnodes,\hedges),\hnode)$}
\label{algo:connect}
\For{$\hnode' \in \hnodes$}
{
    $\alpha \gets {\tt Common\_Positions}(\hnode,\hnode')$\;
    \If{$|\alpha| \geq \nrob$}
    {
        \If{ ${\tt Can\_Assign}(poses,\hnode,\hnode')$}
        {
            $\hedges \gets \hedges \cup (\hnode,\hnode')$\;
        }
    }
}
\end{algorithm}

%$count \gets$ array of zeroes\;
%\For{$p \in {\tt Positions}(\hnode)$}
%{
%    \For{$\hnode' \in {\tt In\_Nodes}(p)$}
%    {
%        $count[\hnode']$++\;
%    }
%}
%\For{$\hnode' \in \hnodes$}
%{
%    \If{$count[n'] \geq \nrob$}
%    {
%        $poses \gets {\tt Common\_Positions}(\hnode,\hnode')$\;
%        \If{ ${\tt Can\_Assign}(poses,\hnode)$ and ${\tt Can\_Assign}(poses,\hnode')$ }
%        {
%            $\hedges \gets \hedges \cup (\hnode,\hnode')$\;
%        }
%    }
%}
%$\hnodes \gets \hnodes \cup \hnode$\;





==> algo_create_hypernode.tex <==
\begin{algorithm}[ht]
\caption{${\tt CREATE\_HYPERNODES} (\graph, \safe, \nrob, \nblank)$}
\label{algo:create_hypernode}
$\pumped \gets {\tt CREATE\_PEBBLE\_GRAPH}(\graph, \safe, \nrob, \nblank)$\;
$\signs \gets {\tt Generate\_Signatures}(\pumped)$\;
$\hnodes \gets \emptyset$\;
\For{$\sign \in \signs$}
{
    $\hnodes \gets \hnodes \cup (\pumped, \sign)$\;
}
${\tt test\_set\_connection}( \hnodes )$\;
return $\hnodes$\;
\end{algorithm}



==> algo_expand_node.tex <==
\begin{algorithm}[ht]
\caption{${\tt EXPAND\_NODE} (\graph, \hnodes, \hnode, \safe)$}
\label{algo:expand}
$R \gets \emptyset$\;
$\pumped \gets {\tt CREATE\_PUMPED}(\graph, \hnodes, \hnode, \safe)$\;
$\Sigma \gets {\tt Compute\_Signatures}(\pumped)$\;
\For{$\sigma \in \Sigma$}
{
    $R \gets R \cup (\pumped, \sigma)$\;
}
return $R$\;
\end{algorithm}



==> algo_manip_prm.tex <==
\begin{algorithm}[ht]
\caption{${\tt ARRANGE\_PRM} ($iterations $m, \safe)$}
\label{algo:arrange_prm}
%Have to create the manipulation part
$\grnodes \gets \emptyset;$ $\gredges \gets \emptyset$ $\frnodes \gets \safe$ $\fredges \gets \emptyset$\;
\For{$i \in 1\ ...\ m$}
{
    $\grnodes \gets \grnodes \cup {\tt Generate\_Stable\_Grasp}()$\;
}
\For{$\grnode \in \grnodes$}
{
    $near \gets {\tt multi}$-${\tt NN}(\grnode, \grnodes)$\;
    \For{$\grnode' \in near$}
    {
        \If{${\tt is\_valid}( \local (\grnode, \grnode') )$}
        {
            $\gredges \gets \gredges \cup \local (\grnode, \grnode')$\;
        }
    }
}
%Have to create the transit part
$\frnodes \gets \frnodes \cup {\tt Released\_Configurations}(\grnodes)$\;
%Must create transitions between them
\For{$\frnode \in \frnodes$}
{
    $\grnode' \gets {\tt NN}(\frnode, \grnodes)$\;
    $\gredges \gets \gredges \cup \local(\frnode, \grnode')$\;
    %Connect up the transit part
    $near \gets {\tt multi}$-${\tt NN}(\frnode, \frnodes)$\;
    \For{$\frnode' \in near$}
    {
        \If{${\tt is\_valid}( \local (\frnode, \frnode') )$}
        {
            $\fredges \gets \fredges \cup \local (\frnode, \frnode')$\;
        }
    }
}
return $\graph = (\grnodes \cup \frnodes, \gredges \cup \fredges)$
\end{algorithm}



==> algo_prxpump.tex <==
\begin{algorithm}[ht]
\caption{${\tt PRX\_PUMP} (s, n_{graph}, n_{hyper}, C_{start}, C_{goal})$}
\label{algo:prxpump}
%build the manipulation roadmap
$G \gets {\tt ARRANGE\_PRM}(n_{graph}, s)$\;
$T \gets \emptyset$ $\hnodes \gets \emptyset$ $L \gets \emptyset$\;
%add start and goal states
$\hnodes_{start} \gets {\tt Create\_Initial}(G, \hnodes, C_{start}, s)$\;
$\hnodes \gets \hnodes \cup \hnodes_{start}$\;
$T \gets T \cup ( \hnodes_{start}, \emptyset )$\;
\For{$i = 1\ ..\ n_{hyper}$}
{
    $\hnodes_{goal} \gets {\tt Create\_Goal}$(G, $\hnodes$, $C_{goal}$)\;
    $\hnodes \gets \hnodes \cup \hnodes_{goal}$\;
    $T \gets T \cup ( N_{goal}, \emptyset )$\;
}
%Iterate
\While{ No solution found }
{
    % Select a Tree
    $T_s \gets {\tt Uniform\_Random}(T)$\;
    % Propagate
    $n_s \gets {\tt Uniform\_Random}(T_s)$\;
    $\hnodes' \gets {\tt EXPAND\_NODE}$ (G, $\hnodes$, $n_s$, s)\;
    % For each created thing
    \For{ $n' \in \hnodes'$ }
    {
        %Attempt connections
        $L' \gets {\tt Attempt\_Connection}$ (n', N)\;        
        %\If{ $L' \neq \emptyset$ }
        %{
            %connection succeeds, add the node.
            $\hnodes \gets \hnodes \cup n'$\;
            $L \gets L \cup L'$\;
        %}
    }
}
return $\hgraph = (\hnodes, L)$\;
\end{algorithm}



==> algo_query.tex <==
\begin{algorithm}[ht]
\caption{${\tt QUERY} ( \cquery_{in} = (\config_{start}, \config_{goal}), \hgraph)$}
\label{algo:query}
$\pumped_{start} = (\config_{start},\emptyset)$\;
$\pumped_{goal} = (\config_{goal},\emptyset)$\;
${\tt CONNECT\_NODE}( \hgraph, \pumped_{start} )$\;
${\tt CONNECT\_NODE}( \hgraph, \pumped_{goal} )$\;
$\alpha_{prev} \gets \config_{start}$\;
$\pi \gets {\tt graph\_search}(\hgraph, \pumped_{start}, \pumped_{goal})$\;
\If{$\pi \neq \emptyset$}
{
    $\Pi \gets emptyset$\;
    \For{$\hnode \in \pi$}
    {
        $\alpha_{next} \gets {\tt Get\_Next\_Edge}(\pi, \hnode)$\;
        $\Pi \gets \Pi \cup {\tt Auletta}(\hnode, \alpha_{prev}, \alpha_{next})$\;
        $\alpha_{prev} \gets \Pi.end$\;
    }
    return $\Pi$\;
}
return failure\;

%$\pumped_{start} = (\config_{start},\emptyset)$\;
%$\pumped_{goal} = (\config_{goal},\emptyset)$\;
%${\tt CONNECT\_NODE}( \hgraph, \pumped_{start} )$\;
%${\tt CONNECT\_NODE}( \hgraph, \pumped_{goal} )$\;
%$\pi \gets {\tt graph\_search}(\hgraph, \pumped_{start}, \pumped_{goal})$\;
%\If{$\pi \neq \emptyset$}
%{
%    $\Pi \gets emptyset$\;
%    \For{$\hnode \in \pi$}
%    {
%        $\cquery \gets {\tt Configuration\_Query}(\hnode)$\;
%        $\Pi \gets \Pi \cup {\tt SOLVE\_PATH}(\hnode, \mathbb{C})$\;
%    }
%    return $\Pi$\;
%}
%return failure\;
\end{algorithm}



==> algo_recursive_create_pumped.tex <==
\begin{algorithm}[ht]
\caption{${\tt CREATE\_PUMPED} (G, N, n, s)$}
\label{algo:create_pumped}
$R \gets V \gets {\tt Valid\_Configuration}(n)$\;
$T \gets {\tt Sample\_Node}( G, V )$\;
$E \gets \emptyset$\;
$F \gets \emptyset$\;
\For{pairs $(t, t') \in T \cup V$, $t \neq t'$}
{
    $\pi \gets {\tt Compute\_Cycle\_Path(G, s, t, t', V, T)}$\;
    \If{${\tt is\_valid}(\pi)$}
    {
        $R \gets R \cup \{t,t'\}$\;
        $E \gets E \cup (t,t')$\;
    }
    \Else
    {
    	$O \gets {\tt Compute\_Collisions}(\pi, T \cup V)$\;
    	\If{$|O| < |T|$}
    	{
    		$F \gets F \cup ((t,t'), O)$\;
    	}
    }
}
\While{New edges added to $E$}
{
	\For{$f \in F$}
	{
		\If{${\tt Test\_Feasible}({\tt Endpoints}(f), {\tt Constraints}(f))$}
		{
	        $R \gets R \cup {\tt Endpoints}(f)$\;
			$E \gets E \cup f$\;
			$F \gets F \setminus f$\;
		}
	}
}
\If{$|R| = |V|$ or $R \in N$}
{
    restart\;
}
return $P = (R, E)$\;
\end{algorithm}



==> algo_solve_path.tex <==
\begin{algorithm}[ht]
\caption{${\tt SOLVE\_PATH} (\hnode=(\pumped, \sign), \mathbb{C} = (\config_{s}, \config_{g}))$}
\label{algo:solve}
\If{$\config_{s} = \config_{g}$}
{
    return $\emptyset$\;
}
$\Pi \gets \emptyset$\;
$\config \gets \config_{s}$\;
$\pi \gets  {\tt Constrained\_Auletta}(\config_{s},\config_{g})$\;
\For{$m \in \pi$}
{
    \If{${\tt Feasible}(\config, m)$}
    {
        $\Pi.append( m )$\;
        $\config \gets {\tt Transition}(\config,m)$\;
    }
    \Else
    {
        $\config_{from} \gets \config$\;
        $\config_{to} \gets {\tt Unconstrained\_Configuration}(m)$\;
        $\Pi.append( {\tt SOLVE\_PATH}(\hnode, (\config_{from},\config_{to})))$\; 
        $\Pi.append( m )$\;
        $\config \gets {\tt Transition}(\config, m)$\;
        $\Pi.append( {\tt SOLVE\_PATH}(\config, \config_{g}) )$\;
        return $\Pi$\;
    }
}
return $\Pi$\;
\end{algorithm}



==> arch_peb_create.tex <==

\input{algo_create_pumped}

The method takes advantage of an intelligent method for creating
pumped configurations, outlined in Algorithm \ref{algo:create_pumped}.
First, a random, valid configuration of the objects is sampled, given
the provided signature of node $n$ (Line 1).  Then, using this 
configuration, a set of prospective nodes is sampled from the graph 
(Line 2).  For each pair of these prospective nodes and the existing
configuration pairs (Line 4), a cyclic path is computed (Line 5).  
This path is constructed from the safe position $s$, to $t$, to $t'$, 
and back to $s$.  If this entire path is collision-free assuming that 
there exists an object at all nodes in $T \cup V$ except $t$ and 
$t'$, then the transition between $t$ and $t'$ is valid, and an
edge is added between $t$ and $t'$ (Lines 6-8).  If no new nodes were
added beyond the original configuration, or if the generated pumped
configuration already exists in the graph, the process tries over to
create a valid pumped configuration (lines 9,10).

Each generated pumped configuration will be used, in conjunction with
a signature for that pumped configuration, as a node in a hypergraph,
$\hgraph$.  The nodes in this hypergraph will be connected in order
to solve the overall query from a start configuration to a goal
configuration.  


==> format/format.tex <==
%%% MY PACKAGES
%\usepackage{amsfonts,amssymb,mathrsfs}
%\usepackage{amsfonts,amssymb}
\usepackage{amsmath}
\usepackage{amssymb}
% \usepackage[cspex,bbgreekl]{mathbbol}
\usepackage{wrapfig}
\usepackage{cite}
% \usepackage{xspace}
% \usepackage{subfigure}
% \usepackage{multirow}
% \usepackage[numbers]{natbib}
% %\usepackage[bookmarks=true]{hyperref}
% \usepackage{verbatim}
% \let\chapter\section
\usepackage[vlined,ruled,linesnumbered]{algorithm2e}
% \usepackage{booktabs}

% % %%% WAFR SUGGESTED PACKAGES
% \usepackage{mathptmx}       % selects Times Roman as basic font
% \usepackage{helvet}         % selects Helvetica as sans-serif font
% \usepackage{courier}        % selects Courier as typewriter font
% %\usepackage{type1cm}        % activate if the above 3 fonts are
% %                             % not available on your system
% % %
\usepackage{makeidx}         % allows index generation
\usepackage{graphicx}        % standard LaTeX graphics tool
% %                              % when including figure files
% \usepackage{multicol}        % used for the two-column index
% \usepackage[bottom]{footmisc}% places footnotes at page bottom
\usepackage{url}

% % Can't do this in WAFR 2014, the new format file doesn't allow it to compile
% % %%%% MY PACKAGES AND CHOICES AGAIN
% % \usepackage[compact]{titlesec}
% % \titlespacing{\section}{0pt}{*2}{*2}
% % \titlespacing{\subsection}{0pt}{*1}{*1}
% % \titlespacing{\subsubsection}{0pt}{*0}{*0}

% \setlength{\parskip}{0pt}
% \setlength{\parsep}{0pt}
% \setlength{\topskip}{0pt}
% \setlength{\topmargin}{0pt}
% \setlength{\topsep}{0pt}
% \setlength{\partopsep}{0pt}

% % booktabs space changing so they are more compressed
% % this is for booktabs tables
% %\addtolength\defaultaddspace{-1pt}
% %\addtolength\belowrulesep{-1pt}
% %\addtolength\aboverulesep{-1pt}

% % float space changing so they are more compressed
% \addtolength{\intextsep}{-15pt}
% \addtolength{\textfloatsep}{-15pt}
\usepackage[table]{xcolor}


==> helpful_text/EXTENDED_BACKGROUND.tex <==
Rearrangement planning problems \cite{Ben-Shahar:1998pi, Ota:2004mi}
have been approached from many different perspectives in the robotics
literature.

{\bf Planning amove Movable Obstacles:} A related and important
challenge for mobile systems is the problem of navigation among
movable obstacles (NAMO). Early on it was shown that NAMO is
NP-hard \cite{Wilfong:1988ys} and later on it was confirmed that this
is the case even for simpler instance that involve only unit square
obstacles \cite{Demaine:2000kl}. Due to problem complexity, most
efforts have focused on efficiency \cite{Chen:1991fk,
Nieuwenhuisen:2006nx} and provide completeness results only for
subclasses of the problem \cite{Stilman:2004qa, Stilman:2006oq}. A
probabilistically complete solution for NAMO was eventually
provided \cite{Berg:2008vn}, but it can only be applied to lower
dimensional robots (2-3 DOFS) and corresponds to uninformed brute
force search. More recently, a decision-theoretic framework for NAMO
has also been presented, which deals with the inherence uncertainty in
both perception and control of real robots \cite{Levinh:2012kx}.

An interesting related challenge is the minimum constaint removal
problem, where the goal is to minimize the amount by which constraints
must be displaced to get a feasible path \cite{Hauser:2012ly}. For
this problem any asymptocally optimal solution has recently been
achieved \cite{Hauser2013Minimum-Constraint}but the problem does not
consider negative interactions between obstacles as in the current
setup.

{\bf Manipulation Planning and Grasping:} The focus in this work is on
building solutions for high-DOF robotic arms and solve manipulation
challenges. Such problems can be approached with a multi-modal
``manipulation graph'' abstraction that contains ``transit'' and
``transfer'' paths \cite{Alami:1989uq, Alami:1997fk, Simeon:2004tg}
and which can be constructed through a sampling-based
process \cite{Kavraki1996Probabilistic-R, LaValle2001}. This paper
follows a similar formalization and applies it appropriately to the
case of multiple similar movable objects towards achieving an
efficient solution. The current work is also utilizing asymptotically
optimal sampling-based planners for the computation of the
manipulation graph \cite{Karaman2011Sampling-based-}. Tree-based
sampling-based planners have also been used successfully in the
context of manipulation planning \cite{Berenson:2009hc,
Berenson:2012ij}.

There is also a variety of different approaches for manipulation
planning, which employ heuristic search \cite{Cohen:2010kx} or
optimization methodologies, such as CHOMP \cite{Zucker:2013vn,
King:2013bs}. The focus of the current paper is more on the
combinatorial challenges that arise from reasoning about multiple
objects and not the actual manipulation method. In this process, this
work is making significant use of heuristic search primitives over
sampling-based roadmaps. The output of the current algorithm could
also potentially be integrated with methods like CHOMP to improve the
quality of the computed solution. There is also significant effort
that focuses on identifying appropriate grasps in complex
scenes \cite{Berenson:2007ly, Ciocarlie:2010fu} but the current paper
does not focus on this aspect of the challenge.

The above manipulation efforts deal with moving and grasping
individual objects. Manipulation planning among multiple movable
obstacles has been considered before for ``monotone'' problems where
each obstacle can be moved at most once \cite{Stilman:2007kl,
Mike:2013fv}.  The solution in the current paper can reason about more
complex challenges. Assembly planning is also solving similar
multi-body problems but the focus there is on separating a collection
of parts and typically the robot path is ignored \cite{Wilson:1994fk,
Halperin:2000uq, Sundaram2001Disassembly-Seq}. Another paradigm for
dealing with cluttered scenes involves non-prehensile manipulation,
such as pushing objects \cite{Cosgun:2011cr, Dogar:2011ve}. The
current solution could potentially be extended to include such actions
but the focus in this paper is on grasping primitives.

{\bf Task and Motion Planning:} Rearrangement planning is an instance
of integrated task and motion planning, which can be seen as an
important step towards solving more complex, cognitive challenges in
robotics and especially in
manipulation \cite{Cambon2009A-Hybrid-Approach-,
Hauser2011Randomized-Multi-Modal-,
Kaelbling2012Integrated-Robot}. Such integrated manipulation problems
have been approached through multi-modal roadmap structures before to
deal with the presence of both discrete and continuous
parameters \cite{Bretl:2004ys,Hauser:2010zr,
Hauser2011Randomized-Multi-Modal-}, which is also useful in the
current challenge.

{\bf Multi-robot Motion Planning:} A major motivation for the current
work is to utilize recent progress in multi-robot motion planning
solvers \cite{Berg:2009ve, Luna:2011tg, Wagner:2012cr, Yu:2012dq} in
the context of manipulation planning.  Multi-robot motion planning is
itself a hard problem due to the high-dimensionality introduced from
the presence of multiple moving bodies. Thus, coupled, complete
approaches typically do not scale well with an increased number of
robots, although there are efforts in decreasing the number of
effective degrees of freedom \cite{Aronov:1999nx}. On the other hand,
decoupled methods, such as priority-based schemes \cite{Berg:2005bh}
or velocity tuning \cite{Leroy:1999qf}, trade completeness for
efficiency.

An interesting line of work in algorithmic theory focuses on the
``pebble motion on graphs'' problem, where disticnt pebbles occupy
need to move from an initial to a goal vertex assignment on a
graph \cite{Kornhauser:1984oq}. The unlabeled version of the problem
has also been studied in the literature \cite{Calinescu:2008kl}. It
turns out that testing the feasibility of a ``pebble motion'' problem
can be answered in linear time \cite{Auletta:1999hc, Goraly:2010ij}.
These results from algorithmic theory, integrated with sampling-based
algorithms for motion planning, inspired a recent method for in
continuous representations \cite{Solovey2012k-Color-Multi-R}. This
approach reduces the multi-robot motion planning problem into a
sequence of discrete pebble problems in a manner that is possible for
the algorithm to efficiently transform movements of pebbles into valid
motions of the robots. 

The current paper is motivated by the progress achieved by this recent
multi-robot motion planning work and the results in algorithmic
theory. It aims to take advantge of similar primitives from the
``pebble motion'' problem to solve in rearrangement planning
challenges where objects motions have to also respect manipulation
constraints.

